Optimizing Vehicular Users Association in Urban Mobile Networks

This study aims to optimize vehicular user association to base stations in a mobile network. We propose an efficient heuristic solution that considers the base station average handover frequency, the channel quality indicator, and bandwidth capacity. We evaluate this solution using real-world base station locations from S\~ao Paulo, Brazil, and the SUMO mobility simulator. We compare our approach against a state of the art solution which uses route prediction, maintaining or surpassing the provided quality of service with the same number of handover operations. Additionally, the proposed solution reduces the execution time by more than 80\% compared to an exact method, while achieving optimal solutions.

==> tables/acronyms.tex <==
\begin{table}[!htb]
    \centering
    \caption{Abbreviations and Symbols}
    \label{tbl:acronyms}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{@{}cc@{}}
    \toprule
        % \multicolumn{2}{c}{Abbreviations and Symbols} \\ \midrule
        RSRQ    &    Reference Signal Received Quality        \\
        eNB    &    Evolved Node B         \\
        UE    &    User Equipment        \\
        $b_{ki}$     & Indicates if the UE$_k$ is connected to eNB$_i$         \\
        $h_i$      &    Average handover frequency of eNB$_i$        \\
        $h_{ij}$    &   Average handover frequency between eNB$_i$ and eNB$_j$         \\
        $l_k$    &      Minimum bandwidth requirement of UE$_k$      \\
        $L_i$    &      Maximum bandwidth capacity of eNB$_i$      \\
        $\Theta_{ki}$ &  RSRQ value between $$ $$ \\
        $R_i$    & Radio transmission range of eNB$_i$           \\
        $d_{ki}$    &   Distance between UE$_k$ and eNB$_i$        \\\bottomrule
    \end{tabular}
    }   
\end{table}

==> tables/networkComparison.tex <==
\begin{table*}[!htb]
    \centering
    \caption{Comparative of the different generations of wireless communication technology.}
    \label{tbl:5gcomparison}
    \resizebox{\textwidth}{!}{%
        \begin{tabular}{@{}cccccc@{}}
            \toprule
            Generation & Features                                                                                                              & Speed & Latency (ms)  & Handover                                                         & Limitations                                                                                              \\ \midrule
            1G      & Analog signals, voice message                                                                                          & \textless~2.4 Kbps          & -              & Horizontal                                                       & Low security                                                                                         \\
            2G      & Digital signal, voice messaging, text e images                                                                                    & \textless~64 Kbps           & \textless~1000 & Horizontal                                                       & weak support to Internet service                                                                    \\
            3G      & \begin{tabular}[c]{@{}c@{}}Voice message,\\  Access to home and mobile Internet,\\  Video calls\end{tabular} & \textless~3.1 Mbps          & \textless~500  & \begin{tabular}[c]{@{}c@{}}Horizontal \\ and Vertical\end{tabular} & Slow speed                                                                             \\
            4G      & Greater speed connection                                                                                               & \textless~300 Mbps          & \textless~100  & \begin{tabular}[c]{@{}c@{}}Horizontal \\ and Vertical\end{tabular} & \begin{tabular}[c]{@{}c@{}}Low scalability and connectivity, \\ support to dense networks\end{tabular} \\
            5G      & \begin{tabular}[c]{@{}c@{}}Ubiquitous connection and high speed, \\ scalability, heterogeneous\end{tabular}              & \textgreater~1 Gbps         & \textless~1    & \begin{tabular}[c]{@{}c@{}}Horizontal\\ and Vertical\end{tabular}  & -                                                                                                       \\ \bottomrule
        \end{tabular}
    }
\end{table*}
